Incorporating Experts' Judgment into Machine Learning Models

Machine learning (ML) models have been quite successful in predicting outcomes in many applications. However, in some cases, domain experts might have a judgment about the expected outcome that might conflict with the prediction of ML models. One main reason for this is that the training data might not be totally representative of the population. In this paper, we present a novel framework that aims at leveraging experts' judgment to mitigate the conflict. The underlying idea behind our framework is that we first determine, using a generative adversarial network, the degree of representation of an unlabeled data point in the training data. Then, based on such degree, we correct the \textcolor{black}{machine learning} model's prediction by incorporating the experts' judgment into it, where the higher that aforementioned degree of representation, the less the weight we put on the expert intuition that we add to our corrected output, and vice-versa. We perform multiple numerical experiments on synthetic data as well as two real-world case studies (one from the IT services industry and the other from the financial industry). All results show the effectiveness of our framework; it yields much higher closeness to the experts' judgment with minimal sacrifice in the prediction accuracy, when compared to multiple baseline methods. We also develop a new evaluation metric that combines prediction accuracy with the closeness to experts' judgment. Our framework yields statistically significant results when evaluated on that metric.

==> sections/OLDER_1_introduction.tex <==
\section{Introduction} \label{Introduction}

To learn the inherent diversity of the data, it is important to prepare a large amount of data in many machine learning applications. The recent success of deep learning \cite{goodfellow2016deep,mikolov2013distributed,brown2020language} also has made that the preparation of a large amount of data is necessary to get the performance gain. Nevertheless, obtaining data is still costly, and we still rely on simple machine learning models in many real-world cases. However, the models often do not correspond to domain experts' intuition (e.g., known laws of physics), 
many decision-makers are in difficulty to decide which one is more trustable. For example, in the scenario of an IT service deal, to train a model that helps to predict the win/loss of a deal, the training data is given as a fixed set (i.e., all historical deals). In practice, it is impractical to collect more labeled data within a short time as the data itself solely depends on business progress. Figure \ref{fig:example} shows examples of two deals. Each deal represents a unique IT service with the same specifications such as storage and computing power. The two sub-graphs represent how the actual winning probability varies depending on prices. In deal 1 and 2, when the price goes up, its winning probability goes down at the beginning, which meets sales experts' expectations. However, the winning probability goes up, when the price increases after 40M dollars in the case of deal 1. That does not make sense to experts, but this often happens in reality due to the low confidence in price negotiation when the service is newly launched. When we train a data-driven ML model, the model is likely to learn the wrong relationship between price and winning probability, and, when we rely on the model, the business will fail.

\begin{figure}[b]
\centering
  \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\linewidth]{figures/example1}
    \caption{Deal 1}
  \end{subfigure}
  \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\linewidth]{figures/example2}
    \caption{Deal 2}
  \end{subfigure}
  \vspace{-2mm}
  \caption{Examples of Conflict between Sales Experts and Observed Data. (Y-axis: Winning prob. and X-axis: Price (\$))}
  \label{fig:example}
\end{figure}

One common solution to this problem is to collect more labeled data and hopefully, this issue will no longer exist. This method, however, may not work in some business scenarios as in the previous example. To mitigate the burden, many existing approaches have attempted to incorporate experts' intuition, and they are based on supervised learning algorithms with additional regularization \cite{mann2007simple,druck2008learning},  weak supervision \cite{stewart2017label}, or model-specific constraint-based learning \cite{ben1995monotonicity,sill1998monotonic,duivesteijn2008nearest}. However, when the number of training data is small or the training data is biased, the existing models are still not reliable for predicting the unobserved world.

In this paper, we focus on how to resolve the conflict between the expert intuition and the data-driven models. The main idea is that we build a prediction model to predict for any unlabeled data point, whether its feature(s), that we have some expert intuition on, is part/represented in the training data or not. If it is presented in it, then we can rely on the data-driven model to get the prediction of that new data point. If not, then we should rely on the expert intuition, or perhaps something in between (a weighted prediction using both the data-driven models and the expert intuition prediction). 

Based on the idea above, we propose a ML framework to resolve the conflict by (1) estimating the reliability of the learned data-driven model given a new instance by using our proposed generative adversarial network and (2) correcting the final prediction using our framework. We assume that experts' intuition could be given as a form of function $g: Z \rightarrow Y$, where $Z$ is intuition variables and $Y$ is class labels. For example, $Z$ could be a price and $Y$ could be winning probability in the IT service deal example above. Our proposed generative adversarial network, which we call \mname{} (Experts' Intuition-based GAN), is to predict whether the intuition variable $Z$ is included/represented in the training dataset or not. If it is, then we trust the data-driven model more, which is trained on the entire training dataset, to predict the probability of winning the deal. Otherwise, we leverage a weighted sum between the probability of a data-driven model and the output of the expert intuition. 

We also come up with proposals for new performance metrics, besides the traditional ones related to the prediction accuracy, to account for evaluating the closeness to the expert intuition. To evaluate our framework, we initially generated four different types of synthetic data to see the impact of the different levels of complexity. In addition, the framework was also evaluated in two real-world scenarios: IT service deal and Credit card approval. Experiments on the datasets show that our model yields significant improvement in all of our performance metrics.

% We propose a framework to resolve the conflict between expert intuition and data-driven AI models. The expectation is that with our framework, the model’s output matches the intuition and at the meantime, the impact on the performance is relieved as much as possible. Furthermore, we aim at developing such a framework that is independent of both the model’s structure and intuition. It is worth noting that the correctness of the expert intuition is out of the scope of this work.

% The key to conflict resolving lies in the judgement of when and how much we should rely on the intuition versus data-driven models. Intuitively, if the instance is similar to training data, the model should be more reliable. Otherwise, we may rely more on intuition. The challenge here is how to quantify the similarity of a to-be-predicted instance to training data.

% In general, our proposal for resolving the conflicts between expert intuition and data-driven models uses simple forms of expert intuition. Specifically, we define two such forms as follows: i) An expert intuition, where a prediction can directly be given, ii) A trend for the relationship between some feature(s) and the prediction is given. There are multiple forms of such trend, e.g., monotonically decreasing, monotonically increasing, first-increasing-then-decreasing, and first-decreasing-then-increasing. Our method consists of two major components: i) Similarity quantification of an unlabeled instance to training data, and ii) Merging the data-driven model’s prediction with the simple forms of expert intuition.


